The Expressive Power of Word Embeddings

We seek to better understand the difference in quality of the several publicly released embeddings. We propose several tasks that help to distinguish the characteristics of different embeddings. Our evaluation of sentiment polarity and synonym/antonym relations shows that embeddings are able to capture surprisingly nuanced semantics even in the absence of sentence structure. Moreover, benchmarking the embeddings shows great variance in quality and characteristics of the semantics captured by the tested embeddings. Finally, we show the impact of varying the number of dimensions and the resolution of each dimension on the effective useful features captured by the embedding space. Our contributions highlight the importance of embeddings for NLP tasks and the effect of their quality on the final results.

==> effects_of_scaling.tex <==
\section{The effects of scaling}
Here we present the comparisons of the scaled vs. unscaled embeddings on these different tasks. Since the learning precedure will sometimes lead to unreasonably value in embeddings--probably extreme small value that is close to zero or range differences between different dimensions. Scaling is a good method to avoid such situation and provide normalized result. But how will scaling affect the performance of our classifier? Here is the performance of both scaled and unscaled version of sentiment classifier and the difference seems really minor.
\begin{table}[!htb]
\begin{scriptsize}
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\ Training method & \multicolumn{2}{|c|}{Turian's embedding} & \multicolumn{4}{|c|}{Turian's embedding} \\
\hline
\ Dimension & 50 & 100 & 25 & 50 & 100 & 200 \\
\hline
\ Sentiment & 0.61\% & 0.02\% & -0.77\% & -0.98\% & -0.67\% & -0.23\% \\
\ Male/Female & -1.92\% & -0.55\% & -0.15\% & -3.18\% & -0.52\% & 1.07\% \\
\ Synonym/Antonym & 1.53\% & -3.59\% & -0.82\% & -2.49\% & 1.11\% & 0.08\% \\
\ Single/Plural & 0.75\% & 0.56\% & 0.72\% & -0.32\% & -0.50\% & 0.25\% \\
\ British/US & 0.33\% & -2.10\% & 0.73\% & -0.55\% & 0.10\% & 2.72\% \\
\hline
\end{tabular}

\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\ Training method & \multicolumn{2}{|c|}{Turian's embedding} & \multicolumn{4}{|c|}{Turian's embedding} \\
\hline
\ Dimension & 50 & 100 & 25 & 50 & 100 & 200 \\
\hline
\ Sentiment & 0.56\% & 0.08\% & -0.66\% & -0.37\% & 0.38\% & -0.27\% \\
\ Male/Female & -1.92\% & -0.38\% & 0.22\% & -1.37\% & -0.38\% & 1.31\% \\
\ Synonym/Antonym & -0.23\% & -1.71\% & -0.18\% & -2.24\% & -0.40\% & -1.06\% \\
\ Single/Plural & 0.08\% & 0.74\% & 0.67\% & -0.43\% & -0.69\% & 0.38\% \\
\ British/US & 0.78\% & -1.95\% & -1.32\% & -0.10\% & 0.24\% & 1.76\% \\
\hline
\end{tabular}

\end{center}
\end{scriptsize}
\caption{$\Delta$ F1 score (top) and $\Delta$ Accuracy(bottom) if apply scaling, linear regression model}
\label{linearregressiondelta}
\end{table}

\begin{table}[!htb]
\begin{scriptsize}
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\ Training method & \multicolumn{2}{|c|}{Turian's embedding} & \multicolumn{4}{|c|}{Turian's embedding} \\
\hline
\ Dimension & 50 & 100 & 25 & 50 & 100 & 200 \\
\hline
\ Sentiment & 0.41\% & 1.28\% & -1.16\% & -1.09\% & 0.57\% & -0.18\% \\
\ Male/Female & -1.53\% & -0.63\% & -2.17\% & -1.78\% & 0.45\% & 2.91\% \\
\ Synonym/Antonym & 2.63\% & -2.4\% & -1.91\% & -2.58\% & 0.47\% & -0.02\% \\
\ Single/Plural & 0.34\% & 1.14\% & 1.39\% & -0.44\% & -0.01\% & 1.93\% \\
\ British/US & -0.18\% & -2.91\% & 1.05\% & 2.33\% & 4.0\% & 4.45\\
\hline
\end{tabular}

\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\ Training method & \multicolumn{2}{|c|}{Turian's embedding} & \multicolumn{4}{|c|}{Turian's embedding} \\
\hline
\ Dimension & 50 & 100 & 25 & 50 & 100 & 200 \\
\hline
\ Sentiment & 0.37\% & 0.84\% & -0.79\% & -0.58\% & 0.56\% & 0.2\% \\
\ Male/Female & -2.21\% & -1.02\% & -0.35\% & -0.53\% & 0.4\% & 3.08\% \\
\ Synonym/Antonym & 0.17\% & -1.11\% & -0.23\% & -2.07\% & -0.51\% & -0.48\% \\
\ Single/Plural & -0.04\% & 1.36\% & 1.34\% & -0.66\% & -0.18\% & 2.0\% \\
\ British/US & -0.29\% & -3.27\% & 0.74\% & 2.35\% & 4.02\% & 3.63\% \\
\hline
\end{tabular}
\end{center}
\end{scriptsize}
\caption{$\Delta$ F1 score (top) and $\Delta$ Accuracy(bottom) if apply scaling, SVM linear kernel}
\label{svmlineardelta}
\end{table}

\begin{table}[!htb]
\begin{scriptsize}
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\ Training method & \multicolumn{2}{|c|}{Turian's embedding} & \multicolumn{4}{|c|}{Turian's embedding} \\
\hline
\ Dimension & 50 & 100 & 25 & 50 & 100 & 200 \\
\hline
\ Sentiment & -1.13\% & -1.11\% & 1.5\% & -1.98\% & -1.4\% & -0.35\% \\
\ Male/Female & -3.01\% & 0.25\% & 0.11\% & 1.22\% & -0.52\% & 0.68\% \\
\ Synonym/Antonym & 2.73\% & -4.35\% & -0.62\% & 0.01\% & -0.34\% & 2.8\% \\
\ Single/Plural & 0.25\% & -0.36\% & 1.36\% & -0.42\% & -1.18\% & -0.22\% \\
\ British/US & 0.13\% & -3.28\% & 0.3\% & 0.25\% & -0.43\% & -0.34\% \\
\hline
\end{tabular}

\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\ Training method & \multicolumn{2}{|c|}{Turian's embedding} & \multicolumn{4}{|c|}{Turian's embedding} \\
\hline
\ Dimension & 50 & 100 & 25 & 50 & 100 & 200 \\
\hline
\ Sentiment & -0.37\% & -0.62\% & 0.78\% & -1.73\% & -1.4\% & -0.34\% \\
\ Male/Female & -2.85\% & -0.11\% & 0.11\% & 0.4\% & -0.49\% & 1.33\% \\
\ Synonym/Antonym & 0.45\% & -1.25\% & 0.16\% & -1.1\% & -1.04\% & 0.98\% \\
\ Single/Plural & -0.22\% & -0.17\% & 1.41\% & -0.54\% & -1.34\% & -0.14\% \\
\ British/US & 0.34\% & -2.68\% & 0.05\% & 0.98\% & 0.29\% & -0.25\% \\
\hline
\end{tabular}
\end{center}
\end{scriptsize}
\caption{$\Delta$ F1 score (top) and $\Delta$ Accuracy(bottom) if apply scaling, SVM RBF kernel}
\label{svmrbfdelta}
\end{table}
The difference of accuracy between scaled and unscaled version can be ignored, while some of the F1 score or recall value differs a lot. Unscaled version's recall using RBF kernel will drop a lot due to many small values that is close to zero, which cause floating precision problem when calculating supporting vectors. Generally speaking, scaled version seems more stable.


==> regression_analysis.tex <==
\section{Prediction reliability}
We would like to show that we can even derive some information from basic linear regression model. Here we listed 10 strongest signal in each class when applying SENNA embeddings in each problem.


